Baryogenesis through Asymmetric Reheating in the Mirror Twin Higgs

We present the $\nu\phi$MTH, a Mirror Twin Higgs (MTH) model realizing asymmetric reheating, baryogenesis and twin-baryogenesis through the out-of-equilibrium decay of a right-handed neutrino without any hard $\mathbb{Z}_2$ breaking. The MTH is the simplest Neutral Naturalness solution to the little hierarchy problem and predicts the existence of a twin dark sector related to the Standard Model (SM) by a $\mathbb{Z}_2$ symmetry that is only softly broken by a higher twin Higgs vacuum expectation value. The asymmetric reheating cools the twin sector compared to the visible one, thus evading cosmological bounds on $\Delta N_{\mathrm{eff}}$. The addition of (twin-)colored scalars allows for the generation of the visible baryon asymmetry and, by the virtue of the $\mathbb{Z}_2$ symmetry, also results in the generation of a twin baryon asymmetry. We identify a unique scenario with top-philic couplings for the new scalars that can satisfy all cosmological, proton decay and LHC constraints; yield the observed SM baryon asymmetry; and generate a wide range of possible twin baryon DM fractions, from negligible to unity. The viable regime of the theory contains several hints as to the possible structure of the Twin Higgs UV completion. Our results motivate the search for the rich cosmological and astrophysical signatures of twin baryons, and atomic dark matter more generally, at cosmological, galactic and stellar scales.

==> changelog_v1.tex <==


v1 changelog

DONE: 




TO DO:

~~~~~~~~

insert 
Farina:2016ndq
into intro cite 

Several studies implement hard $\mathbb{Z}_2$ breakings and generate \emph{all} of the observed DM density from a twin baryon asymmetry generated in an out-of-equilibrium decay together with SM baryons, which requires various departures from the minimal MTH spectrum to accommodate DM self-interaction constraints, account for the full DM relic density, and eliminate dark radiation~\cite{Farina:2015uea, Earl:2019wjw, Feng:2020urb, Kilic:2021zqu}.

~~~~~~~~~~~~~~~~

From: Di Liu <diliu@nyu.edu>
Sent: Tuesday, November 14, 2023 11:20:36 AM
To: Linda Yuan <ly.yuan@mail.utoronto.ca>
Subject: your recent paper 2311.06341
 
	
You don't often get email from diliu@nyu.edu. Learn why this is important
	
Dear Zhihan,

I hope this email finds you well! I have been reading with interest your recent paper 2311.06341 on asymmetric reheating in the Twin Higgs model and the 
subsequent baryogenesis. 

I wanted to bring to your attention my paper https://inspirehep.net/literature/1732984, which addresses the Neff issue in the Twin Higgs model. This is achieved 
by introducing the neutrino portal (Portalino) and a pair of the Z_2 symmetric hypercharged scalars within the model.

I hope you will consider citations to this work in your next revision if you find it relevant and appropriate.

Best regards,

Di


~~~~~~~~~~~~~~~~

